C5: Cloned Concurrency Control that Always Keeps Up

Asynchronously replicated primary-backup databases are commonly deployed to improve availability and offload read-only transactions. To both apply replicated writes from the primary and serve read-only transactions, the backups implement a cloned concurrency control protocol. The protocol ensures read-only transactions always return a snapshot of state that previously existed on the primary. This compels the backup to exactly copy the commit order resulting from the primary's concurrency control. Existing cloned concurrency control protocols guarantee this by limiting the backup's parallelism. As a result, the primary's concurrency control executes some workloads with more parallelism than these protocols. In this paper, we prove that this parallelism gap leads to unbounded replication lag, where writes can take arbitrarily long to replicate to the backup and which has led to catastrophic failures in production systems. We then design C5, the first cloned concurrency protocol to provide bounded replication lag. We implement two versions of C5: Our evaluation in MyRocks, a widely deployed database, demonstrates C5 provides bounded replication lag. Our evaluation in Cicada, a recent in-memory database, demonstrates C5 keeps up with even the fastest of primaries.

==> block_scheduling.tex <==
\section{Page-granularity Protocols Cause Unbounded Replication Lag}
\label{sec:page-scheduling}

\noindentparagraph{System Model.} We use the same model as in
Section~\ref{sec:scheduling:proof}.

\noindentparagraph{Definitions \& Assumptions.} We first define a hash function
$h : O \times \mathbb{N}$ where $O$ is the set of all possible operations. Then
we define an \textit{$h$-granularity protocol} as one that guarantees for all
pairs of operations $o_1$ and $o_2$, if $h(o_1) = h(o_2)$ and $o_1$ precedes
$o_2$ in the log, then the backup executes $o_1$ before $o_2$. This is a
generalization of \sysName{}'s row-level protocol, which uses $h(o) = k(o)$
where $k(o) = x$ for operation $w_T[x]$ in transaction $T$.

A \textit{page-granularity protocol} is then defined by letting $h(o) = b(o)$
where $b(o)$ is the index of the page updated by operation $o$. For simplicity,
our notation assumes each operation updates one page. A logical operation
that updates multiple pages can be modeled by splitting it into multiple physical
operations (e.g., by including page IDs in keys).

\fbok{The idea} of the proof below is to construct a workload where the primary
executes with more parallelism than the backup. This is possible in some
concurrency control protocols, where concurrent transactions may update rows
residing on the same page~\cite{oracle19}. Because page-granularity protocols
are efficient, however, the degree to which the primary's parallelism can exceed
the backup's is more limited than when the backup uses a transaction-granularity
protocol. Thus, we require one additional assumption to ensure the primary
executes with sufficient parallelism.

Define $s = \argmax_i \left|\{ o \mid h(o) = i \}\right|$ and $S = \{o \mid h(o)
= s\}$. Recall we defined $e > 0$ and $e \geq d > 0$ as the number of time units
required for the primary and backup's cores to execute an operation in
isolation. The proof below requires $|S| > \left\lceil \frac{e}{d}
\right\rceil$.

Like the assumption that $m > \left\lceil \frac{e}{d} \right\rceil$, this
assumption is reasonable in practice. With a typical cache line size of
\SI{64}{\byte}---more than enough to store a row with two integer columns---and
a typical page size of \SI{4}{\kibi\byte}, 64 rows can be stored on the same
page, each on a different cache line. Thus, again our assumptions will not be
satisfied only if the backup's can execute operations more than $63$ times
faster than the primary.

\begin{thm}
  Assume $m > \left\lceil \frac{e}{d} \right\rceil$ and $|S| > \left\lceil
    \frac{e}{d} \right\rceil$. Then a primary-backup system that uses two-phase
  locking on its primary and a page-granularity protocol on its backup cannot
  guarantee bounded replication lag.
\end{thm}

\begin{proof}
  Assume we have a primary-backup system as described above, and assume to
  contradict that it guarantees bounded replication lag. Then there exists some
  $L$ such that for all $W \in \mathcal{W}$, the system executes all
  transactions in $W$ with replication lag $\leq L$.
  
  We now construct a workload $W \in \mathcal{W}$ that includes at least one
  transaction with replication lag greater than $L$. Let $n =
  \min\left(m,|S|\right)$. By assumption, $n > \left\lceil \frac{e}{d}
  \right\rceil$. The workload comprises a set of $\left\lceil \frac{nL}{nd -
      e}\right\rceil$ transactions of one write each. By assumption, $nd > e$,
  so the number of transactions is well-defined. Define $A$ such that batches of
  $n$ transactions arrive at the primary every $e$ time units, starting at $0$.
  Within each batch, each transaction updates a unique key such that $o \in S$.
  By assumption, $|S| \geq n$.

  No transactions within a batch conflict, and by assumption, $m \geq n$. Thus, the
  primary, using 2PL, executes all transactions in a batch in parallel. For
  convenience, we assign indices to the transactions in the order the
  appear in the primary's log.

  In the first batch of transactions, $f_p(T_0) = \ldots = f_p(T_{n-1}) =
  e$. At this moment, the primary's cores are all idle and the next batch
  arrives. In general, $f_p(T_i) = \left\lfloor\frac{i+n}{n}\right\rfloor e$.

  The backup uses a page-granularity protocol, so by construction, it serially
  executes all writes in the workload. At time $e$, $n$ transactions arrive at
  the backup. It finishes executing $T_0$ at $e+d$, $\ldots$, and $T_{n-1}$ at
  $e + nd$. Since, by assumption, $nd > e$, $T_n$ arrives at the backup before
  it finishes executing $T_{n-1}$, so the backup immediately starts executing
  $T_n$ after $T_{n-1}$. This is also true subsequent batches. In general,
  $f_b(T_i) = e + (i+1)d$.

  We conclude by showing that for the final transaction $T$ in the workload,
  $f_b(T) - f_p(T) > L$, and thus, the assumed system does not guarantee bounded
  replication lag. First, we derive a lower bound on replication lag:
  \begin{equation*}
    e + (i+1)d - \left\lfloor\frac{i+n}{n}\right\rfloor e > i\left(\frac{nd - e}{n}\right)
  \end{equation*}
  Finally, letting $i = \frac{nL}{nd - e}$ yields $L$ on the right.
\end{proof}

The result above shows that if the primary's parallelism is not constrained by
physical limitations, the backup implements a page-granularity protocol, and
some work is done to replicate each operation, then the backup cannot guarantee
bounded replication lag. Again the same is true if the primary uses a faster
concurrency control mechanism or weaker isolation---both accelerate the primary
while the backup's execution remains constrained.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "paper.tex"
%%% End:


==> cicada_evaluation.tex <==
\section{\syscicada{} Evaluation}
\label{sec:cicada-evaluation}

% The coalescing time is not counted against the primary or the backup in calculating performance numbers. To the best of our knowledge, such coalescing is never performed by the backup in existing replication~\cite{mohan1993remote,minhas2011remusdb,oracle2014eagerRep,qin2017replication,zamanian2019activeMem} and \ccc{} systems~\cite{elnikety2004generalized,hong2013kuafu,king1991remote,oracle2001txnscheduler,mysql8writeset,mysqlgroupcommit,mariadb10,oracle2019ggate,wang2017query,verbitski2018aurora,oracle2019adg,antonopoulos2019socrates}. In most cases, coalescing occurs at the primary, but in some distributed databases, a separate node may be responsible for sorting log records from different primary instances~\cite{verbitski2018aurora}. Thus, this choice only makes it more challenging for \syscicada{} to keep up.

Our evaluation explores the following questions:
\begin{enumerate}
\item Does \syscicada{} help engineers avoid potential disasters caused by
  optimizations of realistic workloads? (\S\ref{sec:cicada-evaluation:tpcc})

\item Does \syscicada{} always keep up with the primary? (\S\ref{sec:cicada-evaluation:throughput})

\end{enumerate}

\noindentparagraph{Experimental Setup.} All experiments ran on the same machines as described in Section~\ref{sec:myrocks-evaluation}. The primary's threads and the backup's \scheduler{}, \worker{}s, and \snapshotter{} are all pinned to their own physical cores.

Because logging slows \cicada{}, we compare against \cicada{}'s performance without logging. This performance is an upper bound on that with logging enabled. For \cicada{}, we use the number of threads that yields the best performance. Similarly, for each \ccc{}, we use the best number of \worker{}s. The backup never uses more threads than the primary. 

Unless stated otherwise, we ran experiments five times and report the median. Error bars show the minimum and maximum.

The workloads are the same as described in Section~\ref{sec:myrocks-evaluation}, and we re-implement the baselines in \cicada{} for fair comparison. \todo{Include details about multiple \kuafu{} impls.}

% Where noted, an additional set of closed-loop clients sent read-only
% transactions to the backup. The backup's workers and read-only threads were
% pinned to separate cores.

% \noindentparagraph{Workloads.} We use three workloads. The first is TPC-C~\cite{tpcc}, a standard OLTP benchmark simulating an
% order-entry application.
% We use the new order and payment transactions, and all experiments used a single warehouse.
% The other two, which refer to as insert-only and adversarial, are synthetic. In each, the
% database contains one table with two integer columns, a primary key and its associated value.

% Each transaction in the insert-only workload comprises a variable number of unique inserts. Each transaction in the adversarial workload comprises a variable number of unique inserts and one update; the updates
% in all transactions set one row's value to a random integer, so all transactions
% conflict.

% \noindentparagraph{Baselines.} \kuafu{}~\cite{hong2013kuafu}, a
% state-of-the-art, transaction-granularity \ccc{} protocol, is our baseline.
% \kuafu{}'s protocol is nearly identical to MySQL 8's
% write-set-based parallel replication~\cite{mysql8writeset} and is strictly better than the database-granularity and epoch-based protocols used in earlier versions of MySQL~\cite{mysql,mysqlgroupcommit} and its variants~\cite{mariadb10}.
% For fair comparison, we re-implemented \kuafu{} in \cicada{}.

\subsection{\syscicada{} Prevents Disasters}
\label{sec:cicada-evaluation:tpcc}

\todo{Report \syscicada{} TPC-C results.}

\begin{figure}[t]
  \includegraphics[width=0.8\linewidth]{figs/tpcc.pdf}
  \caption{\todo{Update Figure with \syscicada{} results.}}
  \label{fig:cicada-tpcc}
\end{figure}

\subsection{\syscicada{} Always Keeps Up}
\label{sec:cicada-evaluation:throughput}

To validate that \syscicada{} always keeps up, we measured the primary and \syscicada{}'s throughput using the insert-only and adversarial workloads. The two
are on opposite ends of the contention spectrum: no transactions
conflict in the former, while all do in the latter. We also present \kuafu{}'s results.

% \begin{table}[t]
%   \centering
%   \begin{tabular}{@{}l r r@{}}
%     \toprule
%     & \multicolumn{2}{l}{\textbf{Throughput (Txns/sec)}}\\
%     & \textbf{Primary} & \textbf{Backup} \\
%     \midrule
%     \textbf{\kuafu{}} & \num{40595} & \num{40647} \\
%     \textbf{\syscicada{}} & \num{40318} & \num{40331} \\
%     \bottomrule
%   \end{tabular}
%   \vspace{2mm}
%   \caption{Primary and backup's throughput with the insert workload. \syscicada{}
%     and \kuafu{} fully utilize the backup's worker threads and easily match the
%     primary's parallelism.}
%   \label{tab:insert-workload}
% \end{table}

Because all transactions are non-conflicting, the insert-only workload stresses the primary's concurrency control and backup's \ccc{}. \cicada{} achieves its best performance with transactions of 16 inserts each, which amortizes any per-transaction overhead. On this workload, \cicada{} inserts about 87M rows/s with 20 threads. \syscicada{} and \kuafu{} both keep up. The former commits 99M rows/s with 10 \worker{}s, and the latter 96M rows/s with 12 \worker{}s.

\syscicada{}'s \scheduler{} is its bottleneck. More specifically, its throughput is limited by memory bandwidth as it and the \worker{}s read and modify log records. \jmf{The following sentences are asking for trouble. Don't say them. Instead say that even on a workload designed to expose scheduler bottlenecks, we find that the scheduler is performant enough to keep up. Also, tack this paragraph onto the previous one.} Although this suggests that a \cicada{} primary with more physical cores may cause \syscicada{} to lag, the current \scheduler{} is sufficient. Since the focus of this work is row-granularity execution, we leave investigation into row-granularity scheduling that always keeps up to future work.  

\begin{figure}[t]
  \centering
  \includegraphics[width=0.8\linewidth]{figs/cicada/adversarial_relative.pdf}
  \caption{Backup's throughput relative to the primary's for the adversarial workload.}
  \label{fig:cicada-adversarial}
\end{figure}

Figure~\ref{fig:cicada-adversarial} compares each \ccc{} protocol's performance to \cicada{}'s
on the adversarial workload. We plot the backup's throughput relative to the
primary's median as we vary the number of non-conflicting inserts per transaction from
1 to 128.

Every transaction updates the same row. Despite the high contention,
however, the \cicada{}'s optimistic concurrency control can execute the non-conflicting inserts that precede the conflicting update in parallel.

\syscicada{} mirrors the primary and executes the
non-conflicting inserts in parallel, so it always keeps up. This advantage is especially evident as the number of inserts per transaction increases from 4 to 8. With more parallel work per transaction, \syscicada{} can leverage additional \worker{}s and its relative throughput actually increases.  

On the other hand, the primary's advantage over \kuafu{}
increases with the number of inserts
per transaction. While the primary executes a larger proportion of the transactions in parallel, \kuafu{} must serialize all of them, so its throughput is bounded by that of a single \worker{}. With 128 inserts per transaction, \kuafu{}'s throughput is just \SI{40}{\percent} of the primary's.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "paper"
%%% End:


==> query_fresh.tex <==
\section{Query Fresh Counterexample}
\label{sec:query-fresh}

We briefly review Query Fresh's design. A more detailed
description of its design can be found in the original paper
\cite{wang2017query}. We then show why it does not guarantee bounded replication
lag.

Query Fresh is a \ccc{} protocol for main-memory databases \cite{wang2017query}.
As the primary sends its redo log to the backup, a set of \worker{}s
process it. Read-only transactions execute in a separate set of threads.

Each row in each table is assigned a unique ID. A table in the backup database
comprises three data structures: the relevant entries in the on-disk log, an
in-memory data array, and an in-memory replay array. The data array is indexed
by row ID and contains linked lists of row versions. The replay array is indexed
by row ID and contains, the log offset of the newest version of the
corresponding row that has been processed by \worker{}s.

As the \worker{}s process the log, they update the replay array but do
not copy versions of each row to the data array. Instantiating the backup
database is left to the read-only transaction threads.

To execute a read-only transaction, a thread first reads the low-watermark
version, which is the the maximum database version such that all log entries
with versions less than or equal to it are guaranteed to have been processed by
the \worker{}s. When reading a database row, the read-only
transaction thread traverses the log and copies any necessary versions to the
data array. This lazy replication scheme can be exploited to create arbitrarily
long lag for a transaction.

Consider the following workload: First, a transaction $T$ writes row $k$. Then,
time passes where no transactions read or write $k$ but there are many updates
to other rows. Thus, a long log of changes accumulates. The log can be made
arbitrarily long because Query Fresh does not garbage collect or consolidate the
backup's logs. Finally, another transaction $U$ writes row $k$. If a read-only
transaction executes after $U$'s write to $k$ is reflected in the replay array
but before the low-watermark version is updated, then it must read $T$'s version
of $k$ because its timestamp is less than $U$'s. But because $k$ was never
read or written during this time, $T$'s version of $k$ is not in the data array,
so the read-only transaction thread must traverse the log and copy it into
memory. Because the log between $T$ and $U$'s updates to $k$ can be made
arbitrarily long so can the time required for this traversal.

Because we define $f_b(T)$ to include the processing performed by read-only
transaction threads in lazy \ccc{} protocols, the idea above can be used to
create a workload that exceeds any finite bound on replication lag. Thus, Query
Fresh does not guarantee bounded lag.



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "paper"
%%% End:

